Hierarchical Deep Reinforcement Learning Approach for Multi-Objective Scheduling With Varying Queue Sizes

Multi-objective task scheduling (MOTS) is the task scheduling while optimizing multiple and possibly contradicting constraints. A challenging extension of this problem occurs when every individual task is a multi-objective optimization problem by itself. While deep reinforcement learning (DRL) has been successfully applied to complex sequential problems, its application to the MOTS domain has been stymied by two challenges. The first challenge is the inability of the DRL algorithm to ensure that every item is processed identically regardless of its position in the queue. The second challenge is the need to manage large queues, which results in large neural architectures and long training times. In this study we present MERLIN, a robust, modular and near-optimal DRL-based approach for multi-objective task scheduling. MERLIN applies a hierarchical approach to the MOTS problem by creating one neural network for the processing of individual tasks and another for the scheduling of the overall queue. In addition to being smaller and with shorted training times, the resulting architecture ensures that an item is processed in the same manner regardless of its position in the queue. Additionally, we present a novel approach for efficiently applying DRL-based solutions on very large queues, and demonstrate how we effectively scale MERLIN to process queue sizes that are larger by orders of magnitude than those on which it was trained. Extensive evaluation on multiple queue sizes show that MERLIN outperforms multiple well-known baselines by a large margin (>22%).

==> sections/variable_queue_length.tex <==
\section{Adapting to Changes in Queue Length}
\label{sec:dynamic_handling}
One significant shortcoming of DRL-based solutions to queue management is the network's inability to adapt to changes in the state or action space \cite{schulman2015trust}. 
More specifically, we refer to the fact that the input of the network, and consequently its number of actions, must be of a fixed size. 
This inflexibility leads to two types of problems. First, this could easily lead to sub-optimal solutions, when easy-to-process items having to wait until the first X items are done. For example, as conducted in \cite{mao2016resource} where the $X$ was 100, the $X+1$ item will have to wait till the first $X$ tasks are completed.
Secondly, this inability to infer the learnt logic to larger queue sizes forces researchers to train their DRL-agents on relatively large state representations, a fact that leads to longer running times and difficulties for the deep network to reach convergence.

To address the challenges described above, we propose a novel \textit{hierarchical approach for dynamic queue size scheduling}. 
Given a queue $Q$, we partition it into fixed size subsets of size $n$, where $n$ is also the number of queue items the outer agent $p^o$ is configured to receive as input. 
This partitioning results in $\ceil{\frac{|Q|}{n}}$ sub-queues.
To ensure that all sub-queues are exactly of size $n$, we use padding when needed. Our padding consists of items that are flagged as ``completed'' (i.e., their processing is already complete), which effectively makes our DRL-agent to ignore them.

Once the partitioning into sub-queues is complete, we apply the outer agent $p^o$ on each sub-queue. 
This results in the creation of a selected set of queue-items whose size we denote as $|Q^`|$. 
Next we check to see whether $Q^` \leq n$. 
If that is the case, $Q^`$ is provided as input to $p^o$ and the scheduling process continues as described in Section \ref{sec:proposedMethod}. Otherwise, if $Q^`> n$, we once again partition the current set into $\ceil{\frac{|Q^`|}{n}}$, and continue to do so until we reach an item set of size $n$. 
An illustration of the proposed process is presented in Figure \ref{fig:hierarchial_step}.
\begin{figure}[ht]
    \centering
    \includegraphics[scale = 0.33]{figures/hierarchial_step_2_new.png}
    \caption{An example of two-stage hierarchical state-action reduction process, with trained DRL algorithm on queue with length of four.}
    \label{fig:hierarchial_step}
\end{figure}


